Elementary Logic in Linear Space

First-order logic is typically presented as the study of deduction in a setting with elementary quantification. In this paper, we take another vantage point and conceptualize first-order logic as a linear space that encodes "plausibility". Whereas a deductive perspective emphasizes how (i.e., process), a space perspective emphasizes where (i.e., location). We explore several consequences that a shift in perspective to "signals in space" has for first-order logic, including (1) a notion of proof based on orthogonal decomposition, (2) a method for assigning probabilities to sentences that reflects logical uncertainty, and (3) a "models as boundary" principle that relates the models of a theory to its "size".

==> media/l2space.tex <==
\begin{tikzpicture}[edge from parent/.style={draw,-latex},level/.style={sibling distance=60mm/#1}]
\node [] (z){$\mvhintree(\mvconst^{(0)}_\epsilon) = 1$}
child {
  node (a) {$\mvhintree(\mvconst^{(1)}_{a}) = 1/3$}
  child {
    node (b) {$\mvhintree(\mvconst^{(2)}_{c}) = 1/6$}
      child { node (c) {$\vdots$} } 
      child { node (d) {$\vdots$} }
  }
  child {
    node (g) {$\mvhintree(\mvconst^{(2)}_{d}) = 1/6$}
      child { node (e) {$\vdots$} }
      child { node (f) {$\vdots$} }
  }
}
child {
  node (j) {$\mvhintree(\mvconst^{(1)}_{b}) = 2/3$}
  child {
    node (k) {$\mvhintree(\mvconst^{(2)}_{e}) = 2/9$}
      child { node (m) {$\vdots$} } 
      child { node (n) {$\vdots$} }
  }
  child {
    node (l) {$\mvhintree(\mvconst^{(2)}_{f}) = 4/9$}
      child { node (o) {$\vdots$} }
      child { node (p) {$\vdots$} }
  }
}
;
\end{tikzpicture}

==> media/sandwich.tex <==
\pgfplotsset{xticklabel={\tick},scaled x ticks=false}
\pgfplotsset{plot coordinates/math parser=false}
\pgfplotsset{every axis legend/.append style={at={(1,0.675)}}}
\pgfplotsset{width=9cm, height=5.5cm}
\begin{tikzpicture} 
    \begin{axis}[symbolic x coords={$\psi_a$,$\psi_b$,$\psi_c$,$\psi_d$,$\psi_e$,$\psi_f$}] 
        % Ground truth
        \addplot+[only marks, mark=square] coordinates { 
            ($\psi_a$,1) 
            ($\psi_b$,0) 
            ($\psi_c$,0) 
            ($\psi_d$,1) 
            ($\psi_e$,0) 
            ($\psi_f$,1)};
        % Sound Approximation
        \addplot+[only marks, mark=x] coordinates { 
            ($\psi_a$,1) 
            ($\psi_b$,1) 
            ($\psi_c$,1) 
            ($\psi_d$,1) 
            ($\psi_e$,0) 
            ($\psi_f$,1)};
        % Complete Approximation
        \addplot+[only marks, mark=+] coordinates { 
            ($\psi_a$,0) 
            ($\psi_b$,0) 
            ($\psi_c$,0) 
            ($\psi_d$,1) 
            ($\psi_e$,0) 
            ($\psi_f$,0)};
        \legend{ground truth, sound approximation, complete approximation};
    \end{axis} 
\end{tikzpicture} 
